StarTrek: Combinatorial Variable Selection with False Discovery Rate Control

Variable selection on the large-scale networks has been extensively studied in the literature. While most of the existing methods are limited to the local functionals especially the graph edges, this paper focuses on selecting the discrete hub structures of the networks. Specifically, we propose an inferential method, called StarTrek filter, to select the hub nodes with degrees larger than a certain thresholding level in the high dimensional graphical models and control the false discovery rate (FDR). Discovering hub nodes in the networks is challenging: there is no straightforward statistic for testing the degree of a node due to the combinatorial structures; complicated dependence in the multiple testing problem is hard to characterize and control. In methodology, the StarTrek filter overcomes this by constructing p-values based on the maximum test statistics via the Gaussian multiplier bootstrap. In theory, we show that the StarTrek filter can control the FDR by providing accurate bounds on the approximation errors of the quantile estimation and addressing the dependence structures among the maximal statistics. To this end, we establish novel Cram\'er-type comparison bounds for the high dimensional Gaussian random vectors. Comparing to the Gaussian comparison bound via the Kolmogorov distance established by \citet{chernozhukov2014anti}, our Cram\'er-type comparison bounds establish the relative difference between the distribution functions of two high dimensional Gaussian random vectors. We illustrate the validity of the StarTrek filter in a series of numerical experiments and apply it to the genotype-tissue expression dataset to discover central regulator genes.

==> smile.tex <==
\RequirePackage{bm} 
\RequirePackage{dsfont}
\RequirePackage{algorithm}
\RequirePackage{algorithmic}
\RequirePackage{booktabs}
\RequirePackage{array}
\RequirePackage{enumerate}

\let\hat\widehat
\let\tilde\widetilde
\let\check\widecheck
\def\given{{\,|\,}}
\def\ds{\displaystyle}
\newcommand\wtilde{\stackrel{\sim}{\smash{\mathcal{W}}\rule{0pt}{1.1ex}}}


\newcommand{\nsubp}{_{i=1}^{n}}
\newcommand{\bbone}{\mathbbm{1}}
\newcommand{\maxnorm}[1]{||#1||_{\infty}}
\newcommand{\Zmax}{\maxnorm{Z}}
\newcommand{\Gmax}{\maxnorm{G}}
\newcommand{\Xmax}{\maxnorm{X}}
\newcommand{\Umax}{\maxnorm{U}}
\newcommand{\Vmax}{\maxnorm{V}}
\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}} 
\newcommand\independent{\protect\mathpalette{\protect\independenT}{\perp}} % independence symbol
\usepackage{centernot}
\newcommand{\dependent}{\centernot{\independent}} % Y not indep Xj | X_\noj

% \let\oldemptyset\emptyset
% \let\emptyset\varnothing
\newcommand{\maxdiff}{\Delta_{\infty}}
\newcommand{\zerodiff}{\Delta_{0}}
\newcommand{\RN}[1]{%
  \textup{\uppercase\expandafter{\romannumeral#1}}%
}

\newcommand{\jlmargin}[2]{{\color{red}#1}\marginpar{\color{red}\raggedright\footnotesize[JL]:#2}}
\newcommand{\lzmargin}[2]{{\color{cyan}#1}\marginpar{\color{cyan}\raggedright\footnotesize[LZ]:#2}}

\def\rot#1{\rotatebox{90}{#1}}
\newcommand{\colored}[1]{{\color{black}{#1}}} % revision with red colors  
%\newcommand{\acc}[1]{{\color{black}{#1}}}
\newcommand{\acc}[1]{{#1}}

\newcommand{\rev}[1]{{#1}} % revision with orange colors  LimeGreen
% \setstcolor{red} % set color for soul package: st command

%%%% dlasso commands
% \newcommand{\normal}{\mathcal{N}}
% \def\hat \beta{\widehat{\beta}}
% \def\coh{{\mu}}
\def\hSigma{\hat{\bSigma}}
\def\hsigma{\hat{\sigma}}
% \def\com{{\mu}_{\rm min}}

\newcommand{\debias}{\text{d}}
\newcommand{\tTheta}{\tilde{\bTheta}}
\newcommand{\cTheta}{\breve{\bTheta}}
\newcommand{\dTheta}{\hat{\bTheta}^\debias}
\newcommand{\tdTheta}{\tilde{\bTheta}^\debias}
\newcommand{\sTheta}{\bTheta^\star}
\newcommand{\signal}{\rho}

\newcommand{\fm}{\mathfrak{m}}
\newcommand{\fp}{\mathfrak{p}}
\newcommand{\fq}{\mathfrak{q}}
\newcommand{\discon}{\fp}

\newcommand{\cqt}{\xi}
\newcommand{\smallop}{o_{\mathbb{P}}(1)}
\newcommand{\lammin}{r_0}

\newcommand{\lerr}{\Xi}
\newcommand{\jdeg}{\|\bTheta_{j,-j}\|_0}

\newcommand{\maxof}[2]{\max\left\{#1, #2\right\}}








%----- bold fonts -----%

\newcommand{\ab}{\mathbf{a}}
\newcommand{\bbb}{\mathbf{b}}
\newcommand{\cbb}{\mathbf{c}}
\newcommand{\db}{\mathbf{d}}
\newcommand{\eb}{\mathbf{e}}
\newcommand{\fb}{\mathbf{f}}
\newcommand{\gb}{\mathbf{g}}
\newcommand{\hb}{\mathbf{h}}
\newcommand{\ib}{\mathbf{i}}
\newcommand{\jb}{\mathbf{j}}
\newcommand{\kb}{\mathbf{k}}
\newcommand{\lb}{\mathbf{l}}
\newcommand{\mb}{\mathbf{m}}
\newcommand{\nbb}{\mathbf{n}}
\newcommand{\ob}{\mathbf{o}}
\newcommand{\pb}{\mathbf{p}}
\newcommand{\qb}{\mathbf{q}}
\newcommand{\rb}{\mathbf{r}}
\newcommand{\sbb}{\mathbf{s}}
\newcommand{\tb}{\mathbf{t}}
\newcommand{\ub}{\mathbf{u}}
\newcommand{\vb}{\mathbf{v}}
\newcommand{\wb}{\mathbf{w}}
\newcommand{\xb}{\mathbf{x}}
\newcommand{\yb}{\mathbf{y}}
\newcommand{\zb}{\mathbf{z}}

\newcommand{\ba}{\bm{a}}
\newcommand{\bb}{\bm{b}}
\newcommand{\bc}{\bm{c}}
\newcommand{\bd}{\bm{d}}
\newcommand{\be}{\bm{e}}
\newcommand{\bbf}{\bm{f}}
\newcommand{\bg}{\bm{g}}
\newcommand{\bh}{\bm{h}}
\newcommand{\bi}{\bmf{i}}
\newcommand{\bj}{\bm{j}}
\newcommand{\bk}{\bm{k}}
\newcommand{\bl}{\bm{l}}
\newcommand{\bbm}{\bm{m}}
\newcommand{\bn}{\bm{n}}
\newcommand{\bo}{\bm{o}}
\newcommand{\bp}{\bm{p}}
\newcommand{\bq}{\bm{q}}
\newcommand{\br}{\bm{r}}
\newcommand{\bs}{\bm{s}}
\newcommand{\bt}{\bm{t}}
\newcommand{\bu}{\bm{u}}
\newcommand{\bv}{\bm{v}}
\newcommand{\bw}{\bm{w}}
\newcommand{\bx}{\bm{x}}
\newcommand{\by}{\bm{y}}
\newcommand{\bz}{\bm{z}}




\newcommand{\Ab}{\mathbf{A}}
\newcommand{\Bb}{\mathbf{B}}
\newcommand{\Cb}{\mathbf{C}}
\newcommand{\Db}{\mathbf{D}}
\newcommand{\Eb}{\mathbf{E}}
\newcommand{\Fb}{\mathbf{F}}
\newcommand{\Gb}{\mathbf{G}}
\newcommand{\Hb}{\mathbf{H}}
\newcommand{\Ib}{\mathbf{I}}
\newcommand{\Jb}{\mathbf{J}}
\newcommand{\Kb}{\mathbf{K}}
\newcommand{\Lb}{\mathbf{L}}
\newcommand{\Mb}{\mathbf{M}}
\newcommand{\Nb}{\mathbf{N}}
\newcommand{\Ob}{\mathbf{O}}
\newcommand{\Pb}{\mathbf{P}}
\newcommand{\Qb}{\mathbf{Q}}
\newcommand{\Rb}{\mathbf{R}}
\newcommand{\Sbb}{\mathbf{S}}
\newcommand{\Tb}{\mathbf{T}}
\newcommand{\Ub}{\mathbf{U}}
\newcommand{\Vb}{\mathbf{V}}
\newcommand{\Wb}{\mathbf{W}}
\newcommand{\Xb}{\mathbf{X}}
\newcommand{\Yb}{\mathbf{Y}}
\newcommand{\Zb}{\mathbf{Z}}

\newcommand{\bA}{\bm{A}}
\newcommand{\bB}{\bm{B}}
\newcommand{\bC}{\bm{C}}
\newcommand{\bD}{\bm{D}}
\newcommand{\bE}{\bm{E}}
\newcommand{\bF}{\bm{F}}
\newcommand{\bG}{\bm{G}}
\newcommand{\bH}{\bm{H}}
\newcommand{\bI}{\bm{I}}
\newcommand{\bJ}{\bm{J}}
\newcommand{\bK}{\bm{K}}
\newcommand{\bL}{\bm{L}}
\newcommand{\bM}{\bm{M}}
\newcommand{\bN}{\bm{N}}
\newcommand{\bO}{\bm{O}}
\newcommand{\bP}{\bm{P}}
\newcommand{\bQ}{\bm{Q}}
\newcommand{\bR}{\bm{R}}
\newcommand{\bS}{\bm{S}}
\newcommand{\bT}{\bm{T}}
\newcommand{\bU}{\bm{U}}
\newcommand{\bV}{\bm{V}}
\newcommand{\bW}{\bm{W}}
\newcommand{\bX}{\bm{X}}
\newcommand{\bY}{\bm{Y}}
\newcommand{\bZ}{\bm{Z}}


%----- calligraphic fonts -----%

\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{{\mathcal{S}}}
\newcommand{\cT}{{\mathcal{T}}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}




%----- blackboard bold fonts-----%

\newcommand{\CC}{\mathbb{C}}
\newcommand{\EEE}{\mathbb{E}}
\newcommand{\VV}{\mathbb{V}}
\newcommand{\II}{\mathbb{I}}
\newcommand{\KK}{\mathbb{K}}
\newcommand{\LL}{\mathbb{L}}
\newcommand{\MM}{\mathbb{M}}
\newcommand{\NN}{\mathbb{N}}
\newcommand{\PPP}{\mathbb{P}}
\newcommand{\GG}{\mathbb{G}}
\newcommand{\QQ}{\mathbb{Q}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\SSS}{\mathbb{S}}
\newcommand{\ZZ}{\mathbb{Z}}
\newcommand{\XX}{\mathbb{X}}
\newcommand{\UU}{\mathbb{U}}
\newcommand{\YY}{\mathbb{Y}}
\newcommand{\OOmega}{\mathbb{\Omega}}




%----- bold greek fonts -----%

\newcommand{\balpha}{\bm{\alpha}}
\newcommand{\bbeta}{\bm{\beta}}
\newcommand{\bgamma}{\bm{\gamma}}
\newcommand{\bdelta}{\bm{\delta}}
\newcommand{\bepsilon}{\bm{\epsilon}}
\newcommand{\bvarepsilon}{\bm{\varepsilon}}
\newcommand{\bzeta}{\bm{\zeta}}
\newcommand{\btheta}{\bm{\theta}}
\newcommand{\bvartheta}{\bm{\vartheta}}
\newcommand{\bkappa}{\bm{\kappa}}
\newcommand{\blambda}{\bm{\lambda}}
\newcommand{\bmu}{\bm{\mu}}
\newcommand{\bnu}{\bm{\nu}}
\newcommand{\bxi}{\bm{\xi}}
\newcommand{\bpi}{\bm{\pi}}
\newcommand{\bvarpi}{\bm{\varpi}}
\newcommand{\brho}{\bm{\varrho}}
\newcommand{\bsigma}{\bm{\sigma}}
\newcommand{\bvarsigma}{\bm{\varsigma}}
\newcommand{\btau}{\bm{\tau}}
\newcommand{\bupsilon}{\bm{\upsilon}}
\newcommand{\bphi}{\bm{\phi}}
\newcommand{\bvarphi}{\bm{\varphi}}
\newcommand{\bchi}{\bm{\chi}}
\newcommand{\bpsi}{\bm{\psi}}
\newcommand{\bomega}{\bm{\omega}}

\newcommand{\bGamma}{\bm{\Gamma}}
\newcommand{\bDelta}{\bm{\Delta}}
\newcommand{\bTheta}{\bm{\Theta}}
\newcommand{\bLambda}{\bm{\Lambda}}
\newcommand{\bXi}{\bm{\Xi}}
\newcommand{\bPi}{\bm{\Pi}}
\newcommand{\bSigma}{\bm{\Sigma}}
\newcommand{\bUpsilon}{\bm{\Upsilon}}
\newcommand{\bPhi}{\bm{\Phi}}
\newcommand{\bPsi}{\bm{\Psi}}
\newcommand{\bOmega}{\bm{\Omega}}

%----- Some standard definitions -----%

\newcommand{\argmin}{\mathop{\mathrm{argmin}}}
\newcommand{\argmax}{\mathop{\mathrm{argmax}}}
\newcommand{\minimize}{\mathop{\mathrm{minimize}}}

\newcommand{\sign}{\mathop{\mathrm{sign}}}
\newcommand{\tr}{\mathop{\mathrm{tr}}}

\DeclareMathOperator{\var}{{\rm Var}}
\DeclareMathOperator{\cor}{\rm Corr}
\DeclareMathOperator{\cov}{\rm Cov}
\DeclareMathOperator{\ind}{\mathds{1}}  % Indicator
\newcommand{\indrbr}[1]{\mathds{1}_{\left(#1\right)}}  
\newcommand{\Indrbr}[1]{\mathds{1}{(#1)}}  
\newcommand{\indcbr}[1]{\mathds{1}_{\left\{#1\right\}}}  
% Indicator with round brackets
\newcommand{\smallfrac}[2]{{\textstyle \frac{#1}{#2}}}  
\newcommand*{\zero}{{\bm 0}}
\newcommand*{\one}{{\bm 1}}

\newcommand{\diag}{{\rm diag}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%% Norms

\newcommand{\norm}[1]{||#1||}
\newcommand{\bignorm}[1]{\bigg|\bigg|#1\bigg|\bigg|}
\newcommand{\opnorm}[2]{| \! | \! | #1 | \! | \! |_{{#2}}}

%%%%% Dot product
\newcommand{\dotp}[2]{\langle{#1},{#2}\rangle}

%%%%  brackets
\newcommand{\inner}[2]{\left\langle #1,#2 \right\rangle}
\newcommand{\rbr}[1]{\left(#1\right)} %% round brackets
\newcommand{\sbr}[1]{\left[#1\right]} %% square brackets
\newcommand{\cbr}[1]{\left\{#1\right\}} %% curly brackets
\newcommand{\nbr}[1]{\left\|#1\right\|} %% norm brackets
\newcommand{\abr}[1]{\left|#1\right|} %% absolute value brackets

%%%%%%%%%  Other commands

\newcommand{\mcomment}[1]{\marginpar{\tiny{#1}}}
\newcommand{\fcomment}[1]{\footnote{\tiny{#1}}}
\newcommand{\overbar}[1]{\mkern 1.5mu\overline{\mkern-1.5mu#1\mkern-1.5mu}\mkern 1.5mu}
\newcommand{\ud}{{\,\mathrm{d}}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%----------------------------------- Lu's definitions ------------------------------------%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%----- Probability and Expectation -----%


%%%% below we consider \left, \right to make sure the outermost brackets are large enough
\newcommand{\EE}[1]{\mathbb{E}\left[{#1}\right]} % Expectation
\newcommand{\Ep}[2]{\mathbb{E}_{#1}\left[{#2}\right]} % Expectation with respect to some law
\newcommand{\Ec}[2]{\mathbb{E}\left[{#1}\,|\,{#2}\right]} % Conditional expectation
\newcommand{\Epc}[3]{\mathbb{E}_{#1}\left[{#2}\,|\,{#3}\right]} % Conditional expectation
%%%% used for total law of expectation such that the "|" is large enough
\newcommand{\Ecmid}[2]{\mathbb{E}\left[{#1} \,\middle|\, {#2}\right]} % Conditional expectation 
\newcommand{\Epcmid}[3]{\mathbb{E}_{#1}\left[{#2}\,\middle|\,{#3}\right]} % Conditional expectation


\newcommand{\PP}[1]{\mathbb{P}\left({#1}\right)} % Probability
\newcommand{\Pp}[2]{\mathbb{P}_{#1}\left({#2}\right)} % Probability with respect to some law
\newcommand{\Pc}[2]{\mathbb{P}\left({#1}\,|\, {#2}\right)} % Conditional probability
\newcommand{\Pcmid}[2]{\mathbb{P}\left({#1} \,\middle|\, {#2}\right)} % Conditional expectation 
\newcommand{\Ppc}[3]{\mathbb{P}_{#1}\left({#2}\,|\,{#3}\right)} % Conditional expectation


\newcommand{\Var}[1]{\mathrm{Var}\left({#1}\right)} % Variance
\newcommand{\Varc}[2]{\mathrm{Var}\left({#1}\,|\,{#2}\right)} % Conditional variance
\newcommand{\Varp}[2]{\mathrm{Var}_{#1}\left({#2}\right)} % Variance with respect to some law
\newcommand{\Varpc}[3]{\mathrm{Var}_{#1}\left({#2}\,|\,{#3}\right)} % Conditional expectation
%%%% used for total law of expectation such that the "|" is large enough
\newcommand{\Varcmid}[2]{\mathrm{Var}\left({#1}\,\middle|\, {#2}\right)} % Conditional expectation 



\newcommand{\Cov}[2]{\mathrm{Cov}\left({#1},{#2}\right)} % Covariance
\newcommand{\Covc}[3]{\mathrm{Cov}\left({#1},{#2}\,|\,{#3}\right)} % Conditional covariance
\newcommand{\Covp}[3]{\mathrm{Cov}_{#1}\left({#2},{#3}\right)} % Covariance with respect to some law

%-----  -----%
\newcommand{\redcom}[1]{{\color{red}{#1}}} % comments colored by red
\newcommand{\bluecom}[1]{{\color{blue}{#1}}} % comments colored by blue
\newcommand{\cyancom}[1]{{\color{cyan}{#1}}} % comments colored by cyan


\newcommand{\myrom}[1]{(\romannumeral #1)}
\newcommand{\myRom}[1]{\MakeUppercase{\romannumeral #1}}
